Factorized class $S$ theories and surface defects

It is known that some theories of class $S$ are actually factorized into multiple decoupled nontrivial four-dimensional $N=2$ theories. We propose a way of constructing examples of this phenomenon using the physics of half-BPS surface defects, and check that it works in one simple example: it correctly reproduces a known realization of two copies of $N=2$ superconformal $SU(2)$ QCD, describing this factorized theory as a class $S$ theory of type $A_3$ on a five-punctured sphere with a twist line. Separately, we also present explicit checks that the Coulomb branch of a putative factorized class $S$ theory has the expected product structure, in two examples.

==> latexmkrc <==
@cus_dep_list = (@cus_dep_list, "svg pdf 0 svg2pdf");
sub svg2pdf {
   my $curdir = cwd();
   system("inkscape -D --export-pdf=\"$curdir/$_[0].pdf\" \"$curdir/$_[0].svg\""); }
$pdf_mode = 1;
$pdflatex = 'pdflatex %O -synctex=1 -interaction=nonstopmode %S';

